Search for Dark Matter Annihilation in the Galactic Center with IceCube-79

The Milky Way is expected to be embedded in a halo of dark matter particles, with the highest density in the central region, and decreasing density with the halo-centric radius. Dark matter might be indirectly detectable at Earth through a flux of stable particles generated in dark matter annihilations and peaked in the direction of the Galactic Center. We present a search for an excess flux of muon (anti-) neutrinos from dark matter annihilation in the Galactic Center using the cubic-kilometer-sized IceCube neutrino detector at the South Pole. There, the Galactic Center is always seen above the horizon. Thus, new and dedicated veto techniques against atmospheric muons are required to make the southern hemisphere accessible for IceCube. We used 319.7 live-days of data from IceCube operating in its 79-string configuration during 2010 and 2011. No neutrino excess was found and the final result is compatible with the background. We present upper limits on the self-annihilation cross-section, $\left<\sigma_\mathrm{A} v\right>$, for WIMP masses ranging from 30 GeV up to 10 TeV, assuming cuspy (NFW) and flat-cored (Burkert) dark matter halo profiles, reaching down to $\simeq 4 \cdot 10^{-24}$ cm$^3$ s$^{-1}$, and $\simeq 2.6 \cdot 10^{-23}$ cm$^3$ s$^{-1}$ for the $\nu\overline{\nu}$ channel, respectively.

==> input/ackn_16012014.tex <==
\begin{acknowledgements}

We acknowledge the support from the following agencies:
U.S. National Science Foundation-Office of Polar Programs,
U.S. National Science Foundation-Physics Division,
University of Wisconsin Alumni Research Foundation,
the Grid Laboratory Of Wisconsin (GLOW) grid infrastructure at the University of Wisconsin - Madison, the Open Science Grid (OSG) grid infrastructure;
U.S. Department of Energy, and National Energy Research Scientific Computing Center,
the Louisiana Optical Network Initiative (LONI) grid computing resources;
Natural Sciences and Engineering Research Council of Canada,
WestGrid and Compute/Calcul Canada;
Swedish Research Council,
Swedish Polar Research Secretariat,
Swedish National Infrastructure for Computing (SNIC),
and Knut and Alice Wallenberg Foundation, Sweden;
German Ministry for Education and Research (BMBF),
Deutsche Forschungsgemeinschaft (DFG),
Helmholtz Alliance for Astroparticle Physics (HAP),
Research Department of Plasmas with Complex Interactions (Bochum), Germany;
Fund for Scientific Research (FNRS-FWO),
FWO Odysseus programme,
Flanders Institute to encourage scientific and technological research in industry (IWT),
Belgian Federal Science Policy Office (Belspo);
University of Oxford, United Kingdom;
Marsden Fund, New Zealand;
Australian Research Council;
Japan Society for Promotion of Science (JSPS);
the Swiss National Science Foundation (SNSF), Switzerland;
National Research Foundation of Korea (NRF);
Danish National Research Foundation, Denmark (DNRF)

\end{acknowledgements}


==> input/authors_16012014.tex <==
\author{IceCube Collaboration: M.~G.~Aartsen\thanksref{Adelaide}
\and R.~Abbasi\thanksref{MadisonPAC}
\and M.~Ackermann\thanksref{Zeuthen}
\and J.~Adams\thanksref{Christchurch}
\and J.~A.~Aguilar\thanksref{Geneva}
\and M.~Ahlers\thanksref{MadisonPAC}
\and D.~Altmann\thanksref{Erlangen}
\and C.~Arguelles\thanksref{MadisonPAC}
\and T.~C.~Arlen\thanksref{PennPhys}
\and J.~Auffenberg\thanksref{Aachen}
\and X.~Bai\thanksref{Bartol,a}
\and M.~Baker\thanksref{MadisonPAC}
\and S.~W.~Barwick\thanksref{Irvine}
\and V.~Baum\thanksref{Mainz}
\and R.~Bay\thanksref{Berkeley}
\and J.~J.~Beatty\thanksref{Ohio,OhioAstro}
\and J.~Becker~Tjus\thanksref{Bochum}
\and K.-H.~Becker\thanksref{Wuppertal}
\and S.~BenZvi\thanksref{MadisonPAC}
\and P.~Berghaus\thanksref{Zeuthen}
\and D.~Berley\thanksref{Maryland}
\and E.~Bernardini\thanksref{Zeuthen}
\and A.~Bernhard\thanksref{Munich}
\and D.~Z.~Besson\thanksref{Kansas}
\and G.~Binder\thanksref{LBNL,Berkeley}
\and D.~Bindig\thanksref{Wuppertal}
\and M.~Bissok\thanksref{Aachen}
\and E.~Blaufuss\thanksref{Maryland}
\and J.~Blumenthal\thanksref{Aachen}
\and D.~J.~Boersma\thanksref{Uppsala}
\and C.~Bohm\thanksref{StockholmOKC}
\and D.~Bose\thanksref{SKKU}
\and S.~B\"oser\thanksref{Bonn}
\and O.~Botner\thanksref{Uppsala}
\and L.~Brayeur\thanksref{BrusselsVrije}
\and H.-P.~Bretz\thanksref{Zeuthen}
\and A.~M.~Brown\thanksref{Christchurch}
\and R.~Bruijn\thanksref{Lausanne}
\and J.~Casey\thanksref{Georgia}
\and M.~Casier\thanksref{BrusselsVrije}
\and D.~Chirkin\thanksref{MadisonPAC}
\and A.~Christov\thanksref{Geneva}
\and B.~Christy\thanksref{Maryland}
\and K.~Clark\thanksref{Toronto}
\and L.~Classen\thanksref{Erlangen}
\and F.~Clevermann\thanksref{Dortmund}
\and S.~Coenders\thanksref{Munich}
\and S.~Cohen\thanksref{Lausanne}
\and D.~F.~Cowen\thanksref{PennPhys,PennAstro}
\and A.~H.~Cruz~Silva\thanksref{Zeuthen}
\and M.~Danninger\thanksref{StockholmOKC}
\and J.~Daughhetee\thanksref{Georgia}
\and J.~C.~Davis\thanksref{Ohio}
\and M.~Day\thanksref{MadisonPAC}
\and J.~P.~A.~M.~de~Andr\'e\thanksref{PennPhys}
\and C.~De~Clercq\thanksref{BrusselsVrije}
\and S.~De~Ridder\thanksref{Gent}
\and P.~Desiati\thanksref{MadisonPAC}
\and K.~D.~de~Vries\thanksref{BrusselsVrije}
\and M.~de~With\thanksref{Berlin}
\and T.~DeYoung\thanksref{PennPhys}
\and J.~C.~D{\'\i}az-V\'elez\thanksref{MadisonPAC}
\and M.~Dunkman\thanksref{PennPhys}
\and R.~Eagan\thanksref{PennPhys}
\and B.~Eberhardt\thanksref{Mainz}
\and B.~Eichmann\thanksref{Bochum}
\and J.~Eisch\thanksref{MadisonPAC}
\and S.~Euler\thanksref{Uppsala}
\and P.~A.~Evenson\thanksref{Bartol}
\and O.~Fadiran\thanksref{MadisonPAC}
\and A.~R.~Fazely\thanksref{Southern}
\and A.~Fedynitch\thanksref{Bochum}
\and J.~Feintzeig\thanksref{MadisonPAC}
\and T.~Feusels\thanksref{Gent}
\and K.~Filimonov\thanksref{Berkeley}
\and C.~Finley\thanksref{StockholmOKC}
\and T.~Fischer-Wasels\thanksref{Wuppertal}
\and S.~Flis\thanksref{StockholmOKC}
\and A.~Franckowiak\thanksref{Bonn}
\and K.~Frantzen\thanksref{Dortmund}
\and T.~Fuchs\thanksref{Dortmund}
\and T.~K.~Gaisser\thanksref{Bartol}
\and J.~Gallagher\thanksref{MadisonAstro}
\and L.~Gerhardt\thanksref{LBNL,Berkeley}
\and L.~Gladstone\thanksref{MadisonPAC}
\and T.~Gl\"usenkamp\thanksref{Zeuthen}
\and A.~Goldschmidt\thanksref{LBNL}
\and G.~Golup\thanksref{BrusselsVrije}
\and J.~G.~Gonzalez\thanksref{Bartol}
\and J.~A.~Goodman\thanksref{Maryland}
\and D.~G\'ora\thanksref{Erlangen}
\and D.~T.~Grandmont\thanksref{Edmonton}
\and D.~Grant\thanksref{Edmonton}
\and P.~Gretskov\thanksref{Aachen}
\and J.~C.~Groh\thanksref{PennPhys}
\and A.~Gro{\ss}\thanksref{Munich}
\and C.~Ha\thanksref{LBNL,Berkeley}
\and C.~Haack\thanksref{Aachen}
\and A.~Haj~Ismail\thanksref{Gent}
\and P.~Hallen\thanksref{Aachen}
\and A.~Hallgren\thanksref{Uppsala}
\and F.~Halzen\thanksref{MadisonPAC}
\and K.~Hanson\thanksref{BrusselsLibre}
\and D.~Hebecker\thanksref{Bonn}
\and D.~Heereman\thanksref{BrusselsLibre}
\and D.~Heinen\thanksref{Aachen}
\and K.~Helbing\thanksref{Wuppertal}
\and R.~Hellauer\thanksref{Maryland}
\and S.~Hickford\thanksref{Christchurch}
\and G.~C.~Hill\thanksref{Adelaide}
\and K.~D.~Hoffman\thanksref{Maryland}
\and R.~Hoffmann\thanksref{Wuppertal}
\and A.~Homeier\thanksref{Bonn}
\and K.~Hoshina\thanksref{MadisonPAC,b}
\and F.~Huang\thanksref{PennPhys}
\and W.~Huelsnitz\thanksref{Maryland}
\and P.~O.~Hulth\thanksref{StockholmOKC}
\and K.~Hultqvist\thanksref{StockholmOKC}
\and S.~Hussain\thanksref{Bartol}
\and A.~Ishihara\thanksref{Chiba}
\and E.~Jacobi\thanksref{Zeuthen}
\and J.~Jacobsen\thanksref{MadisonPAC}
\and K.~Jagielski\thanksref{Aachen}
\and G.~S.~Japaridze\thanksref{Atlanta}
\and K.~Jero\thanksref{MadisonPAC}
\and O.~Jlelati\thanksref{Gent}
\and B.~Kaminsky\thanksref{Zeuthen}
\and A.~Kappes\thanksref{Erlangen}
\and T.~Karg\thanksref{Zeuthen}
\and A.~Karle\thanksref{MadisonPAC}
\and M.~Kauer\thanksref{MadisonPAC}
\and J.~L.~Kelley\thanksref{MadisonPAC}
\and J.~Kiryluk\thanksref{StonyBrook}
\and J.~Kl\"as\thanksref{Wuppertal}
\and S.~R.~Klein\thanksref{LBNL,Berkeley}
\and J.-H.~K\"ohne\thanksref{Dortmund}
\and G.~Kohnen\thanksref{Mons}
\and H.~Kolanoski\thanksref{Berlin}
\and L.~K\"opke\thanksref{Mainz}
\and C.~Kopper\thanksref{MadisonPAC}
\and S.~Kopper\thanksref{Wuppertal}
\and D.~J.~Koskinen\thanksref{Copenhagen}
\and M.~Kowalski\thanksref{Bonn}
\and M.~Krasberg\thanksref{MadisonPAC}
\and A.~Kriesten\thanksref{Aachen}
\and K.~Krings\thanksref{Aachen}
\and G.~Kroll\thanksref{Mainz}
\and J.~Kunnen\thanksref{BrusselsVrije}
\and N.~Kurahashi\thanksref{MadisonPAC}
\and T.~Kuwabara\thanksref{Bartol}
\and M.~Labare\thanksref{Gent}
\and H.~Landsman\thanksref{MadisonPAC}
\and M.~J.~Larson\thanksref{Alabama}
\and M.~Lesiak-Bzdak\thanksref{StonyBrook}
\and M.~Leuermann\thanksref{Aachen}
\and J.~Leute\thanksref{Munich}
\and J.~L\"unemann\thanksref{Mainz}
\and O.~Mac{\'\i}as\thanksref{Christchurch}
\and J.~Madsen\thanksref{RiverFalls}
\and G.~Maggi\thanksref{BrusselsVrije}
\and R.~Maruyama\thanksref{MadisonPAC}
\and K.~Mase\thanksref{Chiba}
\and H.~S.~Matis\thanksref{LBNL}
\and F.~McNally\thanksref{MadisonPAC}
\and K.~Meagher\thanksref{Maryland}
\and A.~Meli\thanksref{Gent}
\and M.~Merck\thanksref{MadisonPAC}
\and T.~Meures\thanksref{BrusselsLibre}
\and S.~Miarecki\thanksref{LBNL,Berkeley}
\and E.~Middell\thanksref{Zeuthen}
\and N.~Milke\thanksref{Dortmund}
\and J.~Miller\thanksref{BrusselsVrije}
\and L.~Mohrmann\thanksref{Zeuthen}
\and T.~Montaruli\thanksref{Geneva}
\and R.~Morse\thanksref{MadisonPAC}
\and R.~Nahnhauer\thanksref{Zeuthen}
\and U.~Naumann\thanksref{Wuppertal}
\and H.~Niederhausen\thanksref{StonyBrook}
\and S.~C.~Nowicki\thanksref{Edmonton}
\and D.~R.~Nygren\thanksref{LBNL}
\and A.~Obertacke\thanksref{Wuppertal}
\and S.~Odrowski\thanksref{Edmonton}
\and A.~Olivas\thanksref{Maryland}
\and A.~Omairat\thanksref{Wuppertal}
\and A.~O'Murchadha\thanksref{BrusselsLibre}
\and T.~Palczewski\thanksref{Alabama}
\and L.~Paul\thanksref{Aachen}
\and J.~A.~Pepper\thanksref{Alabama}
\and C.~P\'erez~de~los~Heros\thanksref{Uppsala}
\and C.~Pfendner\thanksref{Ohio}
\and D.~Pieloth\thanksref{Dortmund}
\and E.~Pinat\thanksref{BrusselsLibre}
\and J.~Posselt\thanksref{Wuppertal}
\and P.~B.~Price\thanksref{Berkeley}
\and G.~T.~Przybylski\thanksref{LBNL}
\and M.~Quinnan\thanksref{PennPhys}
\and L.~R\"adel\thanksref{Aachen}
\and M.~Rameez\thanksref{Geneva}
\and K.~Rawlins\thanksref{Anchorage}
\and P.~Redl\thanksref{Maryland}
\and R.~Reimann\thanksref{Aachen}
\and E.~Resconi\thanksref{Munich}
\and W.~Rhode\thanksref{Dortmund}
\and M.~Ribordy\thanksref{Lausanne}
\and M.~Richman\thanksref{Maryland}
\and B.~Riedel\thanksref{MadisonPAC}
\and S.~Robertson\thanksref{Adelaide}
\and J.~P.~Rodrigues\thanksref{MadisonPAC}
\and C.~Rott\thanksref{SKKU}
\and T.~Ruhe\thanksref{Dortmund}
\and B.~Ruzybayev\thanksref{Bartol}
\and D.~Ryckbosch\thanksref{Gent}
\and S.~M.~Saba\thanksref{Bochum}
\and H.-G.~Sander\thanksref{Mainz}
\and M.~Santander\thanksref{MadisonPAC}
\and S.~Sarkar\thanksref{Copenhagen,Oxford}
\and K.~Schatto\thanksref{Mainz}
\and F.~Scheriau\thanksref{Dortmund}
\and T.~Schmidt\thanksref{Maryland}
\and M.~Schmitz\thanksref{Dortmund}
\and S.~Schoenen\thanksref{Aachen}
\and S.~Sch\"oneberg\thanksref{Bochum}
\and A.~Sch\"onwald\thanksref{Zeuthen}
\and A.~Schukraft\thanksref{Aachen}
\and L.~Schulte\thanksref{Bonn}
\and O.~Schulz\thanksref{Munich}
\and D.~Seckel\thanksref{Bartol}
\and Y.~Sestayo\thanksref{Munich}
\and S.~Seunarine\thanksref{RiverFalls}
\and R.~Shanidze\thanksref{Zeuthen}
\and C.~Sheremata\thanksref{Edmonton}
\and M.~W.~E.~Smith\thanksref{PennPhys}
\and D.~Soldin\thanksref{Wuppertal}
\and G.~M.~Spiczak\thanksref{RiverFalls}
\and C.~Spiering\thanksref{Zeuthen}
\and M.~Stamatikos\thanksref{Ohio,c}
\and T.~Stanev\thanksref{Bartol}
\and N.~A.~Stanisha\thanksref{PennPhys}
\and A.~Stasik\thanksref{Bonn}
\and T.~Stezelberger\thanksref{LBNL}
\and R.~G.~Stokstad\thanksref{LBNL}
\and A.~St\"o{\ss}l\thanksref{Zeuthen}
\and E.~A.~Strahler\thanksref{BrusselsVrije}
\and R.~Str\"om\thanksref{Uppsala}
\and N.~L.~Strotjohann\thanksref{Bonn}
\and G.~W.~Sullivan\thanksref{Maryland}
\and H.~Taavola\thanksref{Uppsala}
\and I.~Taboada\thanksref{Georgia}
\and A.~Tamburro\thanksref{Bartol}
\and A.~Tepe\thanksref{Wuppertal}
\and S.~Ter-Antonyan\thanksref{Southern}
\and G.~Te{\v{s}}i\'c\thanksref{PennPhys}
\and S.~Tilav\thanksref{Bartol}
\and P.~A.~Toale\thanksref{Alabama}
\and M.~N.~Tobin\thanksref{MadisonPAC}
\and S.~Toscano\thanksref{MadisonPAC}
\and M.~Tselengidou\thanksref{Erlangen}
\and E.~Unger\thanksref{Bochum}
\and M.~Usner\thanksref{Bonn}
\and S.~Vallecorsa\thanksref{Geneva}
\and N.~van~Eijndhoven\thanksref{BrusselsVrije}
\and J.~van~Santen\thanksref{MadisonPAC}
\and M.~Vehring\thanksref{Aachen}
\and M.~Voge\thanksref{Bonn}
\and M.~Vraeghe\thanksref{Gent}
\and C.~Walck\thanksref{StockholmOKC}
\and M.~Wallraff\thanksref{Aachen}
\and Ch.~Weaver\thanksref{MadisonPAC}
\and M.~Wellons\thanksref{MadisonPAC}
\and C.~Wendt\thanksref{MadisonPAC}
\and S.~Westerhoff\thanksref{MadisonPAC}
\and B.~J.~Whelan\thanksref{Adelaide}
\and N.~Whitehorn\thanksref{MadisonPAC}
\and K.~Wiebe\thanksref{Mainz}
\and C.~H.~Wiebusch\thanksref{Aachen}
\and D.~R.~Williams\thanksref{Alabama}
\and H.~Wissing\thanksref{Maryland}
\and M.~Wolf\thanksref{StockholmOKC}
\and T.~R.~Wood\thanksref{Edmonton}
\and K.~Woschnagg\thanksref{Berkeley}
\and D.~L.~Xu\thanksref{Alabama}
\and X.~W.~Xu\thanksref{Southern}
\and J.~P.~Yanez\thanksref{Zeuthen}
\and G.~Yodh\thanksref{Irvine}
\and S.~Yoshida\thanksref{Chiba}
\and P.~Zarzhitsky\thanksref{Alabama}
\and J.~Ziemann\thanksref{Dortmund}
\and S.~Zierke\thanksref{Aachen}
\and M.~Zoll\thanksref{StockholmOKC}
}
\authorrunning{IceCube Collaboration}
\thankstext{a}{Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\thankstext{b}{Earthquake Research Institute, University of Tokyo, Bunkyo, Tokyo 113-0032, Japan}
\thankstext{c}{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\institute{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany \label{Aachen}
\and School of Chemistry \& Physics, University of Adelaide, Adelaide SA, 5005 Australia \label{Adelaide}
\and Dept.~of Physics and Astronomy, University of Alaska Anchorage, 3211 Providence Dr., Anchorage, AK 99508, USA \label{Anchorage}
\and CTSPS, Clark-Atlanta University, Atlanta, GA 30314, USA \label{Atlanta}
\and School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA \label{Georgia}
\and Dept.~of Physics, Southern University, Baton Rouge, LA 70813, USA \label{Southern}
\and Dept.~of Physics, University of California, Berkeley, CA 94720, USA \label{Berkeley}
\and Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA \label{LBNL}
\and Institut f\"ur Physik, Humboldt-Universit\"at zu Berlin, D-12489 Berlin, Germany \label{Berlin}
\and Fakult\"at f\"ur Physik \& Astronomie, Ruhr-Universit\"at Bochum, D-44780 Bochum, Germany \label{Bochum}
\and Physikalisches Institut, Universit\"at Bonn, Nussallee 12, D-53115 Bonn, Germany \label{Bonn}
\and Universit\'e Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium \label{BrusselsLibre}
\and Vrije Universiteit Brussel, Dienst ELEM, B-1050 Brussels, Belgium \label{BrusselsVrije}
\and Dept.~of Physics, Chiba University, Chiba 263-8522, Japan \label{Chiba}
\and Dept.~of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand \label{Christchurch}
\and Dept.~of Physics, University of Maryland, College Park, MD 20742, USA \label{Maryland}
\and Dept.~of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA \label{Ohio}
\and Dept.~of Astronomy, Ohio State University, Columbus, OH 43210, USA \label{OhioAstro}
\and Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark \label{Copenhagen}
\and Dept.~of Physics, TU Dortmund University, D-44221 Dortmund, Germany \label{Dortmund}
\and Dept.~of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1 \label{Edmonton}
\and Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, D-91058 Erlangen, Germany \label{Erlangen}
\and D\'epartement de physique nucl\'eaire et corpusculaire, Universit\'e de Gen\`eve, CH-1211 Gen\`eve, Switzerland \label{Geneva}
\and Dept.~of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium \label{Gent}
\and Dept.~of Physics and Astronomy, University of California, Irvine, CA 92697, USA \label{Irvine}
\and Laboratory for High Energy Physics, \'Ecole Polytechnique F\'ed\'erale, CH-1015 Lausanne, Switzerland \label{Lausanne}
\and Dept.~of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA \label{Kansas}
\and Dept.~of Astronomy, University of Wisconsin, Madison, WI 53706, USA \label{MadisonAstro}
\and Dept.~of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin, Madison, WI 53706, USA \label{MadisonPAC}
\and Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany \label{Mainz}
\and Universit\'e de Mons, 7000 Mons, Belgium \label{Mons}
\and T.U. Munich, D-85748 Garching, Germany \label{Munich}
\and Bartol Research Institute and Dept.~of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA \label{Bartol}
\and Dept.~of Physics, University of Oxford, 1 Keble Road, Oxford OX1 3NP, UK \label{Oxford}
\and Dept.~of Physics, University of Wisconsin, River Falls, WI 54022, USA \label{RiverFalls}
\and Oskar Klein Centre and Dept.~of Physics, Stockholm University, SE-10691 Stockholm, Sweden \label{StockholmOKC}
\and Dept.~of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA \label{StonyBrook}
\and Dept.~of Physics, Sungkyunkwan University, Suwon 440-746, Korea \label{SKKU}
\and Dept.~of Physics, University of Toronto, Toronto, Ontario, Canada, M5S 1A7 \label{Toronto}
\and Dept.~of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA \label{Alabama}
\and Dept.~of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA \label{PennAstro}
\and Dept.~of Physics, Pennsylvania State University, University Park, PA 16802, USA \label{PennPhys}
\and Dept.~of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden \label{Uppsala}
\and Dept.~of Physics, University of Wuppertal, D-42119 Wuppertal, Germany \label{Wuppertal}
\and DESY, D-15735 Zeuthen, Germany \label{Zeuthen}
}




==> input/authors_18052015.tex <==
\author{IceCube Collaboration: M.~G.~Aartsen\thanksref{Adelaide}
\and K.~Abraham\thanksref{Munich}
\and M.~Ackermann\thanksref{Zeuthen}
\and J.~Adams\thanksref{Christchurch}
\and J.~A.~Aguilar\thanksref{BrusselsLibre}
\and M.~Ahlers\thanksref{MadisonPAC}
\and M.~Ahrens\thanksref{StockholmOKC}
\and D.~Altmann\thanksref{Erlangen}
\and T.~Anderson\thanksref{PennPhys}
\and M.~Archinger\thanksref{Mainz}
\and C.~Arguelles\thanksref{MadisonPAC}
\and T.~C.~Arlen\thanksref{PennPhys}
\and J.~Auffenberg\thanksref{Aachen}
\and X.~Bai\thanksref{SouthDakota}
\and S.~W.~Barwick\thanksref{Irvine}
\and V.~Baum\thanksref{Mainz}
\and R.~Bay\thanksref{Berkeley}
\and J.~J.~Beatty\thanksref{Ohio,OhioAstro}
\and J.~Becker~Tjus\thanksref{Bochum}
\and K.-H.~Becker\thanksref{Wuppertal}
\and E.~Beiser\thanksref{MadisonPAC}
\and S.~BenZvi\thanksref{MadisonPAC}
\and P.~Berghaus\thanksref{Zeuthen}
\and D.~Berley\thanksref{Maryland}
\and E.~Bernardini\thanksref{Zeuthen}
\and A.~Bernhard\thanksref{Munich}
\and D.~Z.~Besson\thanksref{Kansas}
\and G.~Binder\thanksref{LBNL,Berkeley}
\and D.~Bindig\thanksref{Wuppertal}
\and M.~Bissok\thanksref{Aachen}
\and E.~Blaufuss\thanksref{Maryland}
\and J.~Blumenthal\thanksref{Aachen}
\and D.~J.~Boersma\thanksref{Uppsala}
\and C.~Bohm\thanksref{StockholmOKC}
\and M.~B\"orner\thanksref{Dortmund}
\and F.~Bos\thanksref{Bochum}
\and D.~Bose\thanksref{SKKU}
\and S.~B\"oser\thanksref{Mainz}
\and O.~Botner\thanksref{Uppsala}
\and J.~Braun\thanksref{MadisonPAC}
\and L.~Brayeur\thanksref{BrusselsVrije}
\and H.-P.~Bretz\thanksref{Zeuthen}
\and A.~M.~Brown\thanksref{Christchurch}
\and N.~Buzinsky\thanksref{Edmonton}
\and J.~Casey\thanksref{Georgia}
\and M.~Casier\thanksref{BrusselsVrije}
\and E.~Cheung\thanksref{Maryland}
\and D.~Chirkin\thanksref{MadisonPAC}
\and A.~Christov\thanksref{Geneva}
\and B.~Christy\thanksref{Maryland}
\and K.~Clark\thanksref{Toronto}
\and L.~Classen\thanksref{Erlangen}
\and S.~Coenders\thanksref{Munich}
\and D.~F.~Cowen\thanksref{PennPhys,PennAstro}
\and A.~H.~Cruz~Silva\thanksref{Zeuthen}
\and J.~Daughhetee\thanksref{Georgia}
\and J.~C.~Davis\thanksref{Ohio}
\and M.~Day\thanksref{MadisonPAC}
\and J.~P.~A.~M.~de~Andr\'e\thanksref{Michigan}
\and C.~De~Clercq\thanksref{BrusselsVrije}
\and H.~Dembinski\thanksref{Bartol}
\and S.~De~Ridder\thanksref{Gent}
\and P.~Desiati\thanksref{MadisonPAC}
\and K.~D.~de~Vries\thanksref{BrusselsVrije}
\and G.~de~Wasseige\thanksref{BrusselsVrije}
\and M.~de~With\thanksref{Berlin}
\and T.~DeYoung\thanksref{Michigan}
\and J.~C.~D{\'\i}az-V\'elez\thanksref{MadisonPAC}
\and J.~P.~Dumm\thanksref{StockholmOKC}
\and M.~Dunkman\thanksref{PennPhys}
\and R.~Eagan\thanksref{PennPhys}
\and B.~Eberhardt\thanksref{Mainz}
\and T.~Ehrhardt\thanksref{Mainz}
\and B.~Eichmann\thanksref{Bochum}
\and S.~Euler\thanksref{Uppsala}
\and P.~A.~Evenson\thanksref{Bartol}
\and O.~Fadiran\thanksref{MadisonPAC}
\and S.~Fahey\thanksref{MadisonPAC}
\and A.~R.~Fazely\thanksref{Southern}
\and A.~Fedynitch\thanksref{Bochum}
\and J.~Feintzeig\thanksref{MadisonPAC}
\and J.~Felde\thanksref{Maryland}
\and K.~Filimonov\thanksref{Berkeley}
\and C.~Finley\thanksref{StockholmOKC}
\and T.~Fischer-Wasels\thanksref{Wuppertal}
\and S.~Flis\thanksref{StockholmOKC}
\and T.~Fuchs\thanksref{Dortmund}
\and M.~Glagla\thanksref{Aachen}
\and T.~K.~Gaisser\thanksref{Bartol}
\and R.~Gaior\thanksref{Chiba}
\and J.~Gallagher\thanksref{MadisonAstro}
\and L.~Gerhardt\thanksref{LBNL,Berkeley}
\and K.~Ghorbani\thanksref{MadisonPAC}
\and D.~Gier\thanksref{Aachen}
\and L.~Gladstone\thanksref{MadisonPAC}
\and T.~Gl\"usenkamp\thanksref{Zeuthen}
\and A.~Goldschmidt\thanksref{LBNL}
\and G.~Golup\thanksref{BrusselsVrije}
\and J.~G.~Gonzalez\thanksref{Bartol}
\and J.~A.~Goodman\thanksref{Maryland}
\and D.~G\'ora\thanksref{Zeuthen}
\and D.~Grant\thanksref{Edmonton}
\and P.~Gretskov\thanksref{Aachen}
\and J.~C.~Groh\thanksref{PennPhys}
\and A.~Gro{\ss}\thanksref{Munich}
\and C.~Ha\thanksref{LBNL,Berkeley}
\and C.~Haack\thanksref{Aachen}
\and A.~Haj~Ismail\thanksref{Gent}
\and A.~Hallgren\thanksref{Uppsala}
\and F.~Halzen\thanksref{MadisonPAC}
\and B.~Hansmann\thanksref{Aachen}
\and K.~Hanson\thanksref{MadisonPAC}
\and D.~Hebecker\thanksref{Berlin}
\and D.~Heereman\thanksref{BrusselsLibre}
\and K.~Helbing\thanksref{Wuppertal}
\and R.~Hellauer\thanksref{Maryland}
\and D.~Hellwig\thanksref{Aachen}
\and S.~Hickford\thanksref{Wuppertal}
\and J.~Hignight\thanksref{Michigan}
\and G.~C.~Hill\thanksref{Adelaide}
\and K.~D.~Hoffman\thanksref{Maryland}
\and R.~Hoffmann\thanksref{Wuppertal}
\and K.~Holzapfe\thanksref{Munich}
\and A.~Homeier\thanksref{Bonn}
\and K.~Hoshina\thanksref{MadisonPAC,a}
\and F.~Huang\thanksref{PennPhys}
\and M.~Huber\thanksref{Munich}
\and W.~Huelsnitz\thanksref{Maryland}
\and P.~O.~Hulth\thanksref{StockholmOKC}
\and K.~Hultqvist\thanksref{StockholmOKC}
\and S.~In\thanksref{SKKU}
\and A.~Ishihara\thanksref{Chiba}
\and E.~Jacobi\thanksref{Zeuthen}
\and G.~S.~Japaridze\thanksref{Atlanta}
\and K.~Jero\thanksref{MadisonPAC}
\and M.~Jurkovic\thanksref{Munich}
\and B.~Kaminsky\thanksref{Zeuthen}
\and A.~Kappes\thanksref{Erlangen}
\and T.~Karg\thanksref{Zeuthen}
\and A.~Karle\thanksref{MadisonPAC}
\and M.~Kauer\thanksref{MadisonPAC,Yale}
\and A.~Keivani\thanksref{PennPhys}
\and J.~L.~Kelley\thanksref{MadisonPAC}
\and J.~Kemp\thanksref{Aachen}
\and A.~Kheirandish\thanksref{MadisonPAC}
\and J.~Kiryluk\thanksref{StonyBrook}
\and J.~Kl\"as\thanksref{Wuppertal}
\and S.~R.~Klein\thanksref{LBNL,Berkeley}
\and G.~Kohnen\thanksref{Mons}
\and H.~Kolanoski\thanksref{Berlin}
\and R.~Konietz\thanksref{Aachen}
\and A.~Koob\thanksref{Aachen}
\and L.~K\"opke\thanksref{Mainz}
\and C.~Kopper\thanksref{Edmonton}
\and S.~Kopper\thanksref{Wuppertal}
\and D.~J.~Koskinen\thanksref{Copenhagen}
\and M.~Kowalski\thanksref{Berlin,Zeuthen}
\and K.~Krings\thanksref{Munich}
\and G.~Kroll\thanksref{Mainz}
\and M.~Kroll\thanksref{Bochum}
\and J.~Kunnen\thanksref{BrusselsVrije}
\and N.~Kurahashi\thanksref{Drexel}
\and T.~Kuwabara\thanksref{Chiba}
\and M.~Labare\thanksref{Gent}
\and J.~L.~Lanfranchi\thanksref{PennPhys}
\and M.~J.~Larson\thanksref{Copenhagen}
\and M.~Lesiak-Bzdak\thanksref{StonyBrook}
\and M.~Leuermann\thanksref{Aachen}
\and J.~Leuner\thanksref{Aachen}
\and J.~L\"unemann\thanksref{Mainz}
\and J.~Madsen\thanksref{RiverFalls}
\and G.~Maggi\thanksref{BrusselsVrije}
\and K.~B.~M.~Mahn\thanksref{Michigan}
\and R.~Maruyama\thanksref{Yale}
\and K.~Mase\thanksref{Chiba}
\and H.~S.~Matis\thanksref{LBNL}
\and R.~Maunu\thanksref{Maryland}
\and F.~McNally\thanksref{MadisonPAC}
\and K.~Meagher\thanksref{BrusselsLibre}
\and M.~Medici\thanksref{Copenhagen}
\and A.~Meli\thanksref{Gent}
\and T.~Menne\thanksref{Dortmund}
\and G.~Merino\thanksref{MadisonPAC}
\and T.~Meures\thanksref{BrusselsLibre}
\and S.~Miarecki\thanksref{LBNL,Berkeley}
\and E.~Middell\thanksref{Zeuthen}
\and E.~Middlemas\thanksref{MadisonPAC}
\and J.~Miller\thanksref{BrusselsVrije}
\and L.~Mohrmann\thanksref{Zeuthen}
\and T.~Montaruli\thanksref{Geneva}
\and R.~Morse\thanksref{MadisonPAC}
\and R.~Nahnhauer\thanksref{Zeuthen}
\and U.~Naumann\thanksref{Wuppertal}
\and H.~Niederhausen\thanksref{StonyBrook}
\and S.~C.~Nowicki\thanksref{Edmonton}
\and D.~R.~Nygren\thanksref{LBNL}
\and A.~Obertacke\thanksref{Wuppertal}
\and A.~Olivas\thanksref{Maryland}
\and A.~Omairat\thanksref{Wuppertal}
\and A.~O'Murchadha\thanksref{BrusselsLibre}
\and T.~Palczewski\thanksref{Alabama}
\and L.~Paul\thanksref{Aachen}
\and J.~A.~Pepper\thanksref{Alabama}
\and C.~P\'erez~de~los~Heros\thanksref{Uppsala}
\and C.~Pfendner\thanksref{Ohio}
\and D.~Pieloth\thanksref{Dortmund}
\and E.~Pinat\thanksref{BrusselsLibre}
\and J.~Posselt\thanksref{Wuppertal}
\and P.~B.~Price\thanksref{Berkeley}
\and G.~T.~Przybylski\thanksref{LBNL}
\and J.~P\"utz\thanksref{Aachen}
\and M.~Quinnan\thanksref{PennPhys}
\and L.~R\"adel\thanksref{Aachen}
\and M.~Rameez\thanksref{Geneva}
\and K.~Rawlins\thanksref{Anchorage}
\and P.~Redl\thanksref{Maryland}
\and R.~Reimann\thanksref{Aachen}
\and M.~Relich\thanksref{Chiba}
\and E.~Resconi\thanksref{Munich}
\and W.~Rhode\thanksref{Dortmund}
\and M.~Richman\thanksref{Drexel}
\and S.~Richter\thanksref{MadisonPAC}
\and B.~Riedel\thanksref{Edmonton}
\and S.~Robertson\thanksref{Adelaide}
\and M.~Rongen\thanksref{Aachen}
\and C.~Rott\thanksref{SKKU}
\and T.~Ruhe\thanksref{Dortmund}
\and B.~Ruzybayev\thanksref{Bartol}
\and D.~Ryckbosch\thanksref{Gent}
\and S.~M.~Saba\thanksref{Bochum}
\and L.~Sabbatini\thanksref{MadisonPAC}
\and H.-G.~Sander\thanksref{Mainz}
\and A.~Sandrock\thanksref{Dortmund}
\and J.~Sandroos\thanksref{Copenhagen}
\and S.~Sarkar\thanksref{Copenhagen,Oxford}
\and K.~Schatto\thanksref{Mainz}
\and F.~Scheriau\thanksref{Dortmund}
\and M.~Schimp\thanksref{Aachen}
\and T.~Schmidt\thanksref{Maryland}
\and M.~Schmitz\thanksref{Dortmund}
\and S.~Schoenen\thanksref{Aachen}
\and S.~Sch\"oneberg\thanksref{Bochum}
\and A.~Sch\"onwald\thanksref{Zeuthen}
\and A.~Schukraft\thanksref{Aachen}
\and L.~Schulte\thanksref{Bonn}
\and D.~Seckel\thanksref{Bartol}
\and S.~Seunarine\thanksref{RiverFalls}
\and R.~Shanidze\thanksref{Zeuthen}
\and M.~W.~E.~Smith\thanksref{PennPhys}
\and D.~Soldin\thanksref{Wuppertal}
\and G.~M.~Spiczak\thanksref{RiverFalls}
\and C.~Spiering\thanksref{Zeuthen}
\and M.~Stahlberg\thanksref{Aachen}
\and M.~Stamatikos\thanksref{Ohio,b}
\and T.~Stanev\thanksref{Bartol}
\and N.~A.~Stanisha\thanksref{PennPhys}
\and A.~Stasik\thanksref{Zeuthen}
\and T.~Stezelberger\thanksref{LBNL}
\and R.~G.~Stokstad\thanksref{LBNL}
\and A.~St\"o{\ss}l\thanksref{Zeuthen}
\and E.~A.~Strahler\thanksref{BrusselsVrije}
\and R.~Str\"om\thanksref{Uppsala}
\and N.~L.~Strotjohann\thanksref{Zeuthen}
\and G.~W.~Sullivan\thanksref{Maryland}
\and M.~Sutherland\thanksref{Ohio}
\and H.~Taavola\thanksref{Uppsala}
\and I.~Taboada\thanksref{Georgia}
\and S.~Ter-Antonyan\thanksref{Southern}
\and A.~Terliuk\thanksref{Zeuthen}
\and G.~Te{\v{s}}i\'c\thanksref{PennPhys}
\and S.~Tilav\thanksref{Bartol}
\and P.~A.~Toale\thanksref{Alabama}
\and M.~N.~Tobin\thanksref{MadisonPAC}
\and D.~Tosi\thanksref{MadisonPAC}
\and M.~Tselengidou\thanksref{Erlangen}
\and E.~Unger\thanksref{Uppsala}
\and M.~Usner\thanksref{Zeuthen}
\and S.~Vallecorsa\thanksref{Geneva}
\and N.~van~Eijndhoven\thanksref{BrusselsVrije}
\and J.~Vandenbroucke\thanksref{MadisonPAC}
\and J.~van~Santen\thanksref{MadisonPAC}
\and S.~Vanheule\thanksref{Gent}
\and J.~Veenkamp\thanksref{Munich}
\and M.~Vehring\thanksref{Aachen}
\and M.~Voge\thanksref{Bonn}
\and M.~Vraeghe\thanksref{Gent}
\and C.~Walck\thanksref{StockholmOKC}
\and M.~Wallraff\thanksref{Aachen}
\and N.~Wandkowsky\thanksref{MadisonPAC}
\and Ch.~Weaver\thanksref{MadisonPAC}
\and C.~Wendt\thanksref{MadisonPAC}
\and S.~Westerhoff\thanksref{MadisonPAC}
\and B.~J.~Whelan\thanksref{Adelaide}
\and N.~Whitehorn\thanksref{MadisonPAC}
\and C.~Wichary\thanksref{Aachen}
\and K.~Wiebe\thanksref{Mainz}
\and C.~H.~Wiebusch\thanksref{Aachen}
\and L.~Wille\thanksref{MadisonPAC}
\and D.~R.~Williams\thanksref{Alabama}
\and H.~Wissing\thanksref{Maryland}
\and M.~Wolf\thanksref{StockholmOKC}
\and T.~R.~Wood\thanksref{Edmonton}
\and K.~Woschnagg\thanksref{Berkeley}
\and D.~L.~Xu\thanksref{Alabama}
\and X.~W.~Xu\thanksref{Southern}
\and Y.~Xu\thanksref{StonyBrook}
\and J.~P.~Yanez\thanksref{Zeuthen}
\and G.~Yodh\thanksref{Irvine}
\and S.~Yoshida\thanksref{Chiba}
\and P.~Zarzhitsky\thanksref{Alabama}
\and M.~Zoll\thanksref{StockholmOKC}
}
\authorrunning{IceCube Collaboration}
\thankstext{a}{Earthquake Research Institute, University of Tokyo, Bunkyo, Tokyo 113-0032, Japan}
\thankstext{b}{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\institute{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany \label{Aachen}
\and School of Chemistry \& Physics, University of Adelaide, Adelaide SA, 5005 Australia \label{Adelaide}
\and Dept.~of Physics and Astronomy, University of Alaska Anchorage, 3211 Providence Dr., Anchorage, AK 99508, USA \label{Anchorage}
\and CTSPS, Clark-Atlanta University, Atlanta, GA 30314, USA \label{Atlanta}
\and School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA \label{Georgia}
\and Dept.~of Physics, Southern University, Baton Rouge, LA 70813, USA \label{Southern}
\and Dept.~of Physics, University of California, Berkeley, CA 94720, USA \label{Berkeley}
\and Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA \label{LBNL}
\and Institut f\"ur Physik, Humboldt-Universit\"at zu Berlin, D-12489 Berlin, Germany \label{Berlin}
\and Fakult\"at f\"ur Physik \& Astronomie, Ruhr-Universit\"at Bochum, D-44780 Bochum, Germany \label{Bochum}
\and Physikalisches Institut, Universit\"at Bonn, Nussallee 12, D-53115 Bonn, Germany \label{Bonn}
\and Universit\'e Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium \label{BrusselsLibre}
\and Vrije Universiteit Brussel, Dienst ELEM, B-1050 Brussels, Belgium \label{BrusselsVrije}
\and Dept.~of Physics, Chiba University, Chiba 263-8522, Japan \label{Chiba}
\and Dept.~of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand \label{Christchurch}
\and Dept.~of Physics, University of Maryland, College Park, MD 20742, USA \label{Maryland}
\and Dept.~of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA \label{Ohio}
\and Dept.~of Astronomy, Ohio State University, Columbus, OH 43210, USA \label{OhioAstro}
\and Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark \label{Copenhagen}
\and Dept.~of Physics, TU Dortmund University, D-44221 Dortmund, Germany \label{Dortmund}
\and Dept.~of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA \label{Michigan}
\and Dept.~of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1 \label{Edmonton}
\and Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, D-91058 Erlangen, Germany \label{Erlangen}
\and D\'epartement de physique nucl\'eaire et corpusculaire, Universit\'e de Gen\`eve, CH-1211 Gen\`eve, Switzerland \label{Geneva}
\and Dept.~of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium \label{Gent}
\and Dept.~of Physics and Astronomy, University of California, Irvine, CA 92697, USA \label{Irvine}
\and Dept.~of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA \label{Kansas}
\and Dept.~of Astronomy, University of Wisconsin, Madison, WI 53706, USA \label{MadisonAstro}
\and Dept.~of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin, Madison, WI 53706, USA \label{MadisonPAC}
\and Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany \label{Mainz}
\and Universit\'e de Mons, 7000 Mons, Belgium \label{Mons}
\and Technische Universit\"at M\"unchen, D-85748 Garching, Germany \label{Munich}
\and Bartol Research Institute and Dept.~of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA \label{Bartol}
\and Department of Physics, Yale University, New Haven, CT 06520, USA \label{Yale}
\and Dept.~of Physics, University of Oxford, 1 Keble Road, Oxford OX1 3NP, UK \label{Oxford}
\and Dept.~of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA \label{Drexel}
\and Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA \label{SouthDakota}
\and Dept.~of Physics, University of Wisconsin, River Falls, WI 54022, USA \label{RiverFalls}
\and Oskar Klein Centre and Dept.~of Physics, Stockholm University, SE-10691 Stockholm, Sweden \label{StockholmOKC}
\and Dept.~of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA \label{StonyBrook}
\and Dept.~of Physics, Sungkyunkwan University, Suwon 440-746, Korea \label{SKKU}
\and Dept.~of Physics, University of Toronto, Toronto, Ontario, Canada, M5S 1A7 \label{Toronto}
\and Dept.~of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA \label{Alabama}
\and Dept.~of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA \label{PennAstro}
\and Dept.~of Physics, Pennsylvania State University, University Park, PA 16802, USA \label{PennPhys}
\and Dept.~of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden \label{Uppsala}
\and Dept.~of Physics, University of Wuppertal, D-42119 Wuppertal, Germany \label{Wuppertal}
\and DESY, D-15735 Zeuthen, Germany \label{Zeuthen}
} 

